Treebanking User-Generated Content: a UD Based Overview of Guidelines, Corpora and Unified Recommendations

This article presents a discussion on the main linguistic phenomena which cause difficulties in the analysis of user-generated texts found on the web and in social media, and proposes a set of annotation guidelines for their treatment within the Universal Dependencies (UD) framework of syntactic analysis. Given on the one hand the increasing number of treebanks featuring user-generated content, and its somewhat inconsistent treatment in these resources on the other, the aim of this article is twofold: (1) to provide a condensed, though comprehensive, overview of such treebanks -- based on available literature -- along with their main features and a comparative analysis of their annotation criteria, and (2) to propose a set of tentative UD-based annotation guidelines, to promote consistent treatment of the particular phenomena found in these types of texts. The overarching goal of this article is to provide a common framework for researchers interested in developing similar resources in UD, thus promoting cross-linguistic consistency, which is a principle that has always been central to the spirit of UD.

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = main_LRE_UD_SocMedia
# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles =  
#ellipsis.tex Linguistics.tex















#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).pdf 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
	
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	rm -f $(latexfile).toc
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex &


up:
	git pull

co:	commit
	
commit:
	git commit -m "update" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up

cp: 
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/PapiersEnCours/$(latexfile)_draft.pdf

ebib:
	open $(latexfile).bib





==> notes.tex <==
\section{Editing}
Here's some \hl{examples} for using the proofing \draftreplace{macro}{style}.
A good way to use it is to add notes\draftnote{like that}.
When something need to be \draftHL{absolutely fixed}{Fix me}.\draftadd{Something I added.}\\
\redHL{Fix me!}. \draftremove{Some useless texts.}

\draftnote{Maybe we should anchor the next items list within the work previously done characterizing them?}


\section{Discussion}
Things to discuss:\TL{Is this section going to be split into two (POS vs deps) or for each point are we going to differentiate between annotation type?}
\begin{enumerate}
    \item unit of analysis: sentence \textit{vs} whole message (most commonly a tweet)\\
    we decided not to break the tweet content based on typical sentence boundaries; the rationale behind this was that parsers should ideally be able to parse the whole tweet, not just single sentences, and their output should be directly used for downstream applications. On the other hand, the tweets in our collection were retrieved before the character limit doubled to 280. \\
    C: Because of the shortness of the tweet also each single sentence within it can be often very short and therefore more difficult to be interpreted out of the context provided by the whole tweet. 
    \ines{Practical reasons for segmentation of tweets into sentence-like units: shorter units are much easier to display / annotate, no need to scroll, less time needed for manual annotation}
    \Ale{In the case of twittirò-ud, which also entails a fine-grained annotation for irony, and in which the tweets are all under the former 140 char limit we decided to work at a tweet level and NOT to split sentences because we wanted to analyze the syntactic / semantic relationship among different sentences and ironic triggers (which could be found in two juxtaposed sentences)} 
    C. In general the splitting at tweet level is motivated by a pragmatics and semantics oriented perspective.
    \TL{Code-switching motivation for keeping tweet level (from this paper https://www.aclweb.org/anthology/W19-6905.pdf ) \\INTER-sentential -- Ma tá AON Gaeilge agat úsáid í! It’s Irish Language Week.
‘If you speak ANY Irish, use it! It’s Irish Language Week.’\\
INTER Bilingual -- 'Happy St Patrick’s Day! La Fhéile Pádraig sona daoibh!'}
    
    
    \item tokenization\\
     % !!! Cristina, remember to cite and reference the on-going discussion on the UD official webpage/blog to point out WE ARE aware that's an open issue !!
    in PoSTWITA there are mostly genuine tokenization errors due to missing spaces between words in the original text; UD core group has recently added some recommendations for such cases: \url{https://universaldependencies.org/u/overview/typos.html#wrongly-merged-words} just sticking with this seems reasonable to me.\\
    There are however much more complex cases that Djamé already pointed out, first during our call and then posting here the ongoing discussion within the UD group: \url{https://github.com/UniversalDependencies/docs/issues/641}. I lean towards the third option proposed there by Christopher Manning, i.e. split traditional contractions (e.g. don't/can't in English, "amalgames" in French and Italian\footnote{An exception to this is the case of preposition+article contraction used for partitives: in Italian we consistently leave it unsplit; in French a common decision has to be reached, see \url{https://github.com/UniversalDependencies/docs/issues/644} }, verb-clitic contactions in Italian,... other languages?), but leave unsplit the other ones (LMAO, TFW, etc., fall under this category). As regards LOL, for example, there seems to be a consensus in treating it as an interjection. We also considered  interjections TVTB (\textit{ti voglio tanto bene}, "I love you so much"\footnote{used in Italian to express affection, rather than passionate love}) and WTF.
    % !! Remember to cite and reference the on-going discussion on the UD official webpage/blog to point out WE ARE aware that's an open issue !!
    
    \ines{I agree and that's what we did in our data. Has anybody else problems with splitted compounds? e.g. Japanurlaub (holidays in Japan) vs. Japan Urlaub.} 
    
    \ines{Another case are German particle verbs where the verb particle can be separated, depending on the sentence structure but should be merged with the verb when both are adjacent (e.g. wo das ganze Geld hin geht "where the whole money goes to" should be {\em hingeht}}
    
    \Ale{I agree with the 3rd option too.}
    
    \oz{German UD also splits preposition+article contractions. It is sometimes counterintuitive, e.g., \textit{zum} in \textit{zum Beispiel} is never used as \textit{zu dem Beispiel}, we split it nevertheless.} \Ale{It happens also in Italian.}
    
    \Djame{In principle, I agree with the Manning 3rd option but how about cases where using interjection would render the sentence verbless while there's obviously one:\\
    \textit{idk which one pisses me off the most: Trump or Bolsinaro!}\\}
    
    \manu{Form Blodgett et al: When possible, we used the principle of annotating according to the root of the sub- tree of the original phrase -- I woud vote for this}
    
    
    \item elliptical structures and missing elements\\
    M: in PoSTWITA we basically found three cases of ellipsis: 
    \begin{itemize}
        \item function word/copula ellipsis: not a real problem with UD, imo
        \item predicate ellipsis: it can be treated using orphan
        \item ellipsis due to truncated tweet: often partially or completely unintelligible, a generic dep relation is then used
        \item \ines{omission of main verb for German particle verbs (verb particle can be separated from the main verb; main verb is missing, only verb particle is there (e.g. Ich war nach 10 Stunden endlich durch "I was after 10 hours finally through" should be \textit{durchkommen} to get through).  }
        \item \ines{There are some predicate ellipses where it's unclear what the main verb is. E.g. in "Thiago auf Müller und es steht 2:0" `Tiago to Müller and it's 2:0' it's not clear whether the 'missing' verb would be a specific one out of kick, head,or pass. }
    \end{itemize}
    
    \item domain-specific issues:
    \begin{itemize}
        \item hashtags\\
         treated differently according to the context in which they occur, i.e. whether syntactically integrated or not: in the second case, parataxis still seems the good solution to me (we also added the sub-type \texttt{parataxis:hashtag}); not sure about the proper UPOS, though; we used SYM, but I'm open to other solutions.
         \oz{We used the real POS for hashtags, e.g. \textit{\#funny} is ADJ. Sometimes a hashtag is a phrase or even a sentence, e.g. \textit{\#SayNoToRacism}. Then we didn't break it, and used X as UPOS. What do you do in such cases?}
         \ines{We do the same: \#Friday/NOUN, \#handsUpItsWeekend/X}
         \TL{We differentiate between intra-sentential hashtags and classifying hashtags. See section 3.1 https://www.aclweb.org/anthology/W15-4301.pdf}
         

         
        \item at-mentions\\
        M: similar to hashtags as regards the different treatment depending on the syntactic context: vocative when used "in isolation", actual syntactic role otherwise. As regards its UPOS, we used SYM, but PROPN is probably more appropriate
        
        \Ale{PROPN seems more appropriate to me too.}
        
        \TL{As per hashtags - Does it not depend on the role of the token?  if it's serving a content role such as SUBJ/OBJ/etc - e.g. "Did anyone see @Hozier on the Late Show last night?" But what if handles are just used to tag someone at the end of a tweet? }
        
        \oz{We anonymised at-mentions as @username, nevertheless used PROPN. The vocative suggestion sounds good when used at the end of a tweet.}
        
        \ines{We also used PROPN.}
        
        \Djame{We also used PROPN, exactly as one would with actual proper-name. Distinction should be done at the functional level -- but I understand this is not always the path followed by UD --}
        
        \item RTs \\
        M: not clear to me how we should treat this; a noun? or rather a verb (with the at-mention that usually follows as obj?)?
        \Ale{To me this, looks like it could be treated as a \texttt{parataxis} element with the \@mention as an \texttt{vocative}.}
        \oz{we gave the POS tag X for them, but I don't have any strong opinion here.}
        \item URLs\\
        M: except for a few cases (at least in our treebank) they are often appended at the end of the tweet and don't seem to bear any linguistic function; we opted for dep and attached them to the root
        \oz{for POS, the UD guidelines suggest SYM, and we followed it.}
        \ines{We used X/dep (I must have overlooked the SYM suggestion but could easily change this to SYM/dep).}
        \item pictograms\\
        M: discourse markers that can be attached to the closest non-projective head
        \Djame{Even when they're used as a verb? \\
        I [heart] pizzas}
        %{\DejaSans I ❤️ pizzas}}
        
        \ines{We also use discourse (POS: SYM) but attach them to the root of the sentence.}
        \item other?
        \item \ines{mark-up (==> $>>$ *** etc.)}
        \item \Ale{How to deal with tweets with new lines? We usually strip the new line and pretend it was never there and consider the wholw tweet as a unique instance. Shall we substitute it with the "\textbackslash{n}" wildcard?) - Shall we split each row as a separate sentence?}
        \oz{I kept them in my corpus with a wildcard because most of the time they function as sentence boundaries.}

    \end{itemize}
   
    \item code mixing\\
    M: expressions longer that one word could be annotated as flat:foreign
    
    \ines{main problem: What to consider as a foreign word? (Ich bin cool/I am cool: German, Ich bin tired/I am tired: code-switching? No clear-cut boundaries...)}
    %%% alex's note moved to buffer.tex (djame)
    %% same with Ozlem's (djame)
    
    
    \Ale{It's true that the boundaries are blurry but I suppose we could put an effort to find a clear-cut definition and an agreement with the languages involved following some principles based on definitions of institutes such as "Accademia della Crusca", and "Deutsche Akademie für Sprache und Dichtung", etc. - distinguishing between 'calques', 'adapted loans', 'not-adapted loans', 'foreign words'\footnote{This link is in Italian and some other language, but not in english. But I think it provides a good classification we could start from: \url{https://it.wikipedia.org/wiki/Prestito_linguistico}.} and then deciding what should be marked as \texttt{foreign} and what not.}


    \oz{There have been blurry cases all the time, this is how languages evolve after all, but with social media the transition is more dynamic. That is, institutions are not able to respond to the change as fast. I'm experiencing this a lot, I ask a large group of native speakers and the majority agrees the (English) word is now considered German, but it is not in dictionaries or on any official page. Should we then consider it non-German?}
    \Djame{In our upcoming Arabizi treebank (North African dialect, code switch with French, 36\% of the vocabulary being French we decided to not discriminate between so-called native words and apparently foreign as they could appear in similar context. We marked them with a feature and keep the annotation going. We tried to maintain some kind of neutral view regarding the syntactic annotation scheme except for cases that only exist in either French or Arabic.}
    
    \item disfluencies\\
    M: not an expert of spoken language processing; we treated some of them as simple interjections (e.g. \textit{beh/ecco}, "well", \textit{ah}, "uh"), consistently with their dictionary definition.
  
    \ines{Often not clear how to distingish interjections (Ahhh!) from similar spoken language phenomena such as hesitation markers (uhm), back-channel signals, responsives etc. (see table below). Often not possible to disambiguate especially without prosody/stress (UGC). I think this shouldn't be part of the UD POS but should be handled in the language-specific annotation schemes (for German proposals have been made how to extend the STTS POS guidelines to deal with spoken language phenomena and UGC.)}
    

 
\begin{table*}[t]
    \centering 
    \begin{tabular}{|l|l|l|l|}
    \hline
     {\bf type}         &               & {\bf example} & {\bf engl. translation}\\ 
     \hline
     interjection       & ahh, uh, Iiih, boah, Mann, Alter & &  \\
     \hline 
     acronyms           & LOL, WTF & & \\
     \hline
     hesitation marker  & uhm, ähm      & {\bf ähm} wie heißt er?   & {\bf uhm} what's his name? \\ 
     \hline
     back-channel signal & mhm, yes, ok  & {\bf mhm}, kenn ich   & {\bf u-hu}, I know it \\ 
     \hline
     responsive         & yes, no, ok, ne,  nö, nee, ok, klar  & {\bf ne}, die nicht & {\bf no}, not her \\
     \hline
     tag question       & ne, oder, right, ok, ja, gell & Du hast Urlaub, {\bf ne}?   & You're on holidays, {\bf right}? \\
    \hline
    discourse marker    & well, also, nun,  allora, naja & & \\
    \hline
    other (interjections,  & thanks, sorry, bye, hello, ahoi, hihihi,   & & \\
    onomatopoeia, ...)     & cheers, pfft, miao, bang           & & \\
    \hline 
    inflectives     & *wink*, *kopf-schüttel*, *facebook-weg-klick* & & \\
    (German only)   & *auf-die-Schulter-{\bf klopf}* & (verb form is uninflected) & on-the-shoulder-pat  \\
    \hline 
    \end{tabular}
 
    \caption{Particles frequently used in spoken discourse and/or in UGC}
    \label{tab:particles}
\end{table*}

 
  
\end{enumerate}
   



%\section{debate on the UD regarding UGC tokenization}
%(ds) hi all, there was a very interesting discussion on the UD mailing list regarding the tokenization of non standard compound like imma, gotcha and complex forms like lol, lmao and the rest. \url{https://github.com/UniversalDependencies/docs/issues/641} Most of the treebanks whose authors decided to not break non canonical compounds are not UD-Kosher. You can have a look to  the "unit of analysis" section at \url{http://www.spmrl.org/sancl-posters2014.html}.



%%%%%FUTURE WORK ??? %%%%%%%
%\section{Multilingual Parsing on Social Media Texts}
%Can we propose some parsing results applied to social media, going beyond those presented for POSTWITA?? Can we discuss cross-lingual transfer parsing considering Italian and French as case study? The goal should be to improve parsing results also for non-standard texts by benefiting from cross-lingual transfer.

\begin{comment}
\subsubsection{Lemmatization} Providing a unique solution with regard to lemmatization is quite hard, because of the different strategies we adopted according to each specific issue that arises from UGC, and that we have discussed individually in the paragraphs above. Here, we try to summarize the different solutions we propose in a short list. 

\vspace{-0.1cm}
\begin{itemize}
    \item{\textit{acronyms and abbreviations}}\\
    $\rightarrow$ leave them as they are (LOL, LMAO, WTF...).
    
    \item{\textit{code-switching}}\\
    $\rightarrow$  leave them as they are.
     
    \begin{examples}
    \item IT: Mario Monti for president?

    \end{examples}
\vspace{-0.1cm}
    
        \begin{footnotesize}
        \begin{dependency}
        \begin{deptext}
        Text: \&[.2cm]\textit{Digitalizzazione} \&[.2cm] \textit{scuola} \&[.2cm] \textbf{\textit{:}} \&[.2cm] \textit{3\%} \&[.2cm] \textbf\textit{loading} \\
        Lemma: \&[.2cm] mario \&[.2cm] monti \&[.2cm] \ul{for} \&[.2cm] \ul{president} \&[.2cm] ? \\
        % UPOS: \&[.2cm] PROPN \&[.2cm] PROPN \&[.2cm] X   \&[.2cm] X         \&[.2cm] ? \\
        % XPOS: \&[.2cm] SP    \&[.2cm] SP    \&[.2cm] EN  \&[.2cm] EN        \&[.2cm] ? \\
        \end{deptext}
        \deproot{2}{\normalsize root}
        \depedge{2}{4}{\normalsize nmod}
        \depedge{4}{5}{\normalsize flat:foreign}
        \depedge[edge unit distance=2.2ex]{2}{6}{\normalsize punct}
        \depedge{2}{3}{\normalsize flat:name}
        \end{dependency}
        \end{footnotesize}
        
    \item{\textit{wrong words due to keyboard's automatic spell-check}}\\
    $\rightarrow$ retrieve the lemma in its standard word form.
    

            
    \item{\textit{hashtags, mentions, emojis}} \\
    $\rightarrow$ if the element has a clear syntactic function, retrieve the lemma in its standard word form as in Example \ref{lemmaheart}, otherwise leave them as they are.
    
        \begin{examples}
        \item EN: I \hspace{0.04cm} \Heart \hspace{0.07cm} you\label{lemmaheart}
        \end{examples}
            
            \begin{footnotesize}
            \begin{dependency}
            \begin{deptext}
            Text:  \&[.2cm] \textit{I} \&[.2cm] \textit{\textbf{\Heart}} \&[.2cm] \textit{you} \\
            Lemma:  \&[.2cm] I \&[.2cm] {\textbf{\ul{love}}} \&[.2cm] you  \\
            % UPOS:  \&[.2cm] PRON \&[.2cm] VERB \&[.2cm] PRON  \\
            % XPOS: \&[.2cm]  PE \&[.2cm]   V  \&[.2cm] PE \&[.2cm]    \\
            \end{deptext}
            \depedge{3}{2}{\normalsize nsubj}
            \deproot[edge unit distance=3ex]{3}{\normalsize root}
            \depedge{3}{4}{\normalsize obj}
            \end{dependency}
            \end{footnotesize}
                
    \item{\textit{contractions and non-standard word forms}}\\
    $\rightarrow$ retrieve the lemma in its standard word form.
    
    %TL have turned this into a figure so that it's easier to centre (it was bleeding into the 2nd column). But if the placement of the example numbering is an issue - then you can undo it - or fix 20 and 21 accordingly?
    

    \begin{examples}
    \item IT: lo so xké è stato dopo sanremo
    \end{examples}\\
    
    
    \begin{footnotesize}    
        \begin{dependency}
        \begin{deptext}
        Text: \&  \textit{lo}	\& \textit{so}	\& \textbf{\textit{xké}}	\& \textit{è}	\& \textit{stato}	\& \textit{dopo}	\& \textit{sanremo}	\\
        Lemma: \&  lo	\& sapere	\& \textbf{\ul{perché}}	\& essere	\& essere	\& dopo	\& sanremo	\\ 
        % UPOS: \&  PRON	\& VERB	\& SCONJ	\& AUX	\& AUX	\& ADP	\& PROPN	\\
        % XPOS: \&  PRON	\& VERB	\& SCONJ	\& AUX	\& AUX	\& ADP	\& PROPN	\\
        \end{deptext}
    
        \depedge{3}{2}{obj}
        \deproot[edge unit distance=4ex]{3}{root}%%
        \depedge{8}{4}{mark}
        \depedge{8}{5}{aux}
        \depedge{8}{6}{cop}
        \depedge{8}{7}{case}
        \depedge{3}{8}{ccomp}
        \end{dependency}
        \end{footnotesize}
        
\end{itemize}
\end{comment}

==> unimorph.tex <==

\paragraph{Treatment of morphology}

Like the UD group, the collaborative Unimorph project \cite{Kirov16,kirov-etal-2018-unimorph,mccarthy-etal-2020-unimorph} is developing a cross-lingual schema for annotating the morphosyntactic details of language. While UD's main focus  is on the annotation of dependency syntactic relations between tokens in corpora of running text, Unimorph focuses on the analysis of morphological features at the word type level.\footnote{Note that in some variants of UD, in addition to overt text tokens, empty nodes are also allowed and these can then enter dependency annotations.} Nevertheless, UD corpora also include finer-grained annotations of lexical and grammatical properties of tokens beyond POS.

The attribute-value pairs used for morphological features in UD's schema are constructed in a bottom-up fashion: features are adapted and newly included as evidence comes in from languages for which resources are created. By contrast, UniMorph is top-down: its design is guided by surveys of the typological literature and aims to be complete, accounting for all attested morphological phenomena. Accordingly, Unimorph provides some attributes that UD lacks, such as ones for information structure and deixis. In other cases, Unimorph provides more values for certain attributes: for instance, it covers 23 different noun classes used by Bantu languages, whereas UD  only provides the values MASC, FEM, NEUT for gender.

In addition, there are differences in the feature syntax employed. For instance, Unimorph uses templatic features (combined of several atoms), which often rely on feature value combinations. UD uses combined values too (e.g. Gender=Masc,Neut) but in UD they expresses disjunction, used when one cannot select just one of the values. Unimorph can capture disjunction too, but it also allows for conjunction of features, or elaboration, e.g. IN+ABL. Especially in the case of locative morphemes, Unimorph combinations of its atomic features may correspond to a single distinct case value in UD.

As reported by \cite{kirov-etal-2018-unimorph}, a preliminary survey of UD annotations shows that approximately 68% of UD features  have direct UniMorph schema equivalents, with these feature sets covering 97.04% of the complete UD tags.\footnote{\cite{mccarthy-etal-2018-marrying} reports on  experiments in which UD feature annotation is deterministically converted to Unimorph format for multiple languages. } As the authors note, some UD features are outside the scope of UniMorph, which marks primarily morphosyntactic and morphosemantic distinctions. For example, UD has markers for abbreviated forms and foreign borrowings, which Unimorph does not provide as it limits its features to those needed for capturing the meanings of overt inflectional morphemes.  Conversely, some Unimorph features are not represented in UD. One reason for this is because relevant languages exhibiting the features in question are not represented among the UD corpora. For instance, the Bantu noun classes are not accounted for in UD because no UD corpora for such languages exist.

While the differences between UD and Unimorph in respect to working procedure and coverage need not forestall future convergence, coming to a single unified representation may still be difficult. One reason is the basic tension between the typology-based features of Unimorph and the features (feature names) chosen by language-experts in UD. 
For  typological interests, a central problem with language-specific terminology is that, cross-linguistically, shared labels often do not represent shared meaning. E.g. a dative case in one language may not necessarily be very similar to a dative case in another \cite{sylak2016composition}. But a semantically consistent definition of dative case may well mean that some cases in specific languages could  no longer be called dative, thereby conflicting with language-specific grammatical traditions. Such differences could most easily be handled by maintaining both the typology-based and the language-particular analyses in parallel. 
Another reason seems to be that the different interests of syntactic and morphological analysis favor different policies in some cases. For instance, while Unimorph initially focused on building  morphological paradigms for nouns, verbs and adjectives, it has recently expanded its scope to function words, which necessitated dealing with syntactic fusions (or contractions)  such as Spanish `del' (de+el) \cite{mccarthy-etal-2020-unimorph}. While UD disassembles such forms into distinct tokens that can enter into dependency relations, Unimorph chose to follow the format of the French Treebank \cite{Abeillé2003} and  separates the annotations into one part for each syntactic unit, joined by a plus sign.
As \cite{mccarthy-etal-2020-unimorph} note, the recognition that lemmas and word forms can be segmented 
opens up possibilities for  morphological dictionaries. And with respect to clitics or agglutinative formations, opens up the possibility to map morphological features onto segments of a word form. While this reasoning is understandable, the resulting policy makes the alignment of current UD and Unimorph harder.



